Learning Non-linguistic Skills without Sacrificing Linguistic Proficiency

The field of Math-NLP has witnessed significant growth in recent years, motivated by the desire to expand LLM performance to the learning of non-linguistic notions (numerals, and subsequently, arithmetic reasoning). However, non-linguistic skill injection typically comes at a cost for LLMs: it leads to catastrophic forgetting of core linguistic skills, a consequence that often remains unaddressed in the literature. As Math-NLP has been able to create LLMs that can closely approximate the mathematical skills of a grade-schooler or the arithmetic reasoning skills of a calculator, the practicality of these models fail if they concomitantly shed their linguistic capabilities. In this work, we take a closer look into the phenomena of catastrophic forgetting as it pertains to LLMs and subsequently offer a novel framework for non-linguistic skill injection for LLMs based on information theoretic interventions and skill-specific losses that enable the learning of strict arithmetic reasoning. Our model outperforms the state-of-the-art both on injected non-linguistic skills and on linguistic knowledge retention, and does so with a fraction of the non-linguistic training data (1/4) and zero additional synthetic linguistic training data.

==> tables/backup.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{@{}lccccc@{}}
\toprule
                          &                       & \multicolumn{4}{c}{Model Accuracy}                                         \\ \midrule
Model                     & Training Samples      & Validation Set & OOD {[}$20^{3}$,$10^{4}${]} & OOD {[}$10^4$,$10^5${]} & OOD {[}$10^5$,$10^6${]} \\ \midrule
GenBERT                   & 165,000 (n)           & \textbf{100\%} & 1.32\%            & 0.06\%            & 0.0\%             \\
BERT                      & \textbf{41,250 (n/4)} & 96.63\%        & 7.20\%            & \textbf{0.12\%}   & 0.0\%             \\
SkillBERT (+ \textit{lreg})       & \textbf{41,250 (n/4)} & 95.67\%        & 9.66\%            & \textbf{0.12\%}   & 0.0\%             \\
SkillBERT (+ \textit{lreg} + \textit{lewc}) & \textbf{41,250 (n/4)} & 98.01\%        & \textbf{19.44\%}  & \textbf{0.12\%}   & 0.0\%             \\ \bottomrule
\end{tabular}
\end{table*}
